Collision Avoidance Verification of Multiagent Systems with Learned Policies

For many multiagent control problems, neural networks (NNs) have enabled promising new capabilities. However, many of these systems lack formal guarantees (e.g., collision avoidance, robustness), which prevents leveraging these advances in safety-critical settings. While there is recent work on formal verification of NN-controlled systems, most existing techniques cannot handle scenarios with more than one agent. To address this research gap, this paper presents a backward reachability-based approach for verifying the collision avoidance properties of Multi-Agent Neural Feedback Loops (MA-NFLs). Given the dynamics models and trained control policies of each agent, the proposed algorithm computes relative backprojection sets by (simultaneously) solving a series of Mixed Integer Linear Programs (MILPs) offline for each pair of agents. We account for state measurement uncertainties, making it well aligned with real-world scenarios. Using those results, the agents can quickly check for collision avoidance online by solving low-dimensional Linear Programs (LPs). We demonstrate the proposed algorithm can verify collision-free properties of a MA-NFL with agents trained to imitate a collision avoidance algorithm (Reciprocal Velocity Obstacles). We further demonstrate the computational scalability of the approach on systems with up to 10 agents.

==> sections/experiments/scaling.tex <==
{\small
    \begin{table}[h]
        \vspace{-1ex}
        \centering
            \begin{tabular}{c|cc|c|cc}
            \hline
            \# agents & RBPOA     & online    & \# agents & RBPOA    & online    \\
                      & [s/pair]  & [ms/pair] &           & [s/pair] & [ms/pair] \\
            \hline
            2  & 201.50 & 1.49 & 7 & 260.43 & 1.38 \\
            3  & 239.46 & 1.39 & 8  & 251.47 & 1.52 \\
            4  & 217.77 & 1.40 & 9  & 300.60 & 1.35 \\
            5  & 201.97 & 1.31 & 10 & 321.68 & 1.60 \\
            6  & 265.23 & 1.59 & \\
            \hline
            \end{tabular}
        \caption{Pair-wise untime computing RBPOA/online safety check of systems with up to 10 agents controlled by vector field policy with [20, 20] hidden neurons.}
        \label{Tab:runtime_MA}
    \end{table}
}%

To demonstrate the scalability of ReBAR-MA, we verify systems with up to 10 agents and report the pair-wise offline and online runtime in \cref{Tab:runtime_MA}. To demonstrate our method's ability to handle larger and more complex NN controllers, we trained the agents with [20,20] hidden neurons, that mimics the vector field policy in \cite{rober2022backward}. Note we do not train the agents to avoid each other. We set $\epsilon = 0.5$ for all experiments. From the table we can see that pair-wise verification runtime does not increase dramatically w.r.t. number of agents and fluctuates between 201.50s to 321.68s, and the online safety check takes 1.31ms to 1.60ms per pair on average. As our approach is parallelizable, we are able to verify a system up to 10 agent in minutes in the ideal case where we compute all RBPOAs in parallel. In the worst case, if we compute all RBPOAs and online safety check sequentially, the total verification runtime will be $\mathcal{O}(n^2)$ the respective average pair-wise runtime. The resulting RBPOA and online safety check for the 10-agent system is shown in \cref{fig:10_agent}. For a 10-agent system, sampling-based methods are inefficient for computing the relative backprojection set, due to the high dimensionality of the input joint state vector. Instead, our RBPOA provides an over approximation to the sampled RBPUA, and identifies unsafe cases online, demonstrating our pair-wise approach's scalability to increasing number of neural network controlled agents.

\begin{figure}[t] 
    \vspace{5pt}
    \captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=0.95\linewidth]{images/experiment/all_rbpoa_of_agent1.png}
    \caption{1 Timestep RBPOA between agent 1 and 2}
    \end{subfigure}%
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=0.95\linewidth]{images/experiment/10_agent_online.png}
    \caption{Successfully identified some starting positions are unsafe}
    \end{subfigure}
    \caption{10 vector field agent system. (a): Overlaid RBPOA of agent 1 and 2-10. (b): unsafe region (red) marked by online safety check identifies sampled unsafe region (blue)}
    \label{fig:10_agent}
    \vspace{-0.1in}
\end{figure} 

==> sections/experiments/two_agent.tex <==
In this section, we demonstrate ReBAR by verifying multi-agent collision avoidance NN controllers trained to mimic the RVO algorithm~\cite{van2008reciprocal}. We collect 1M state-action pairs for agent positions randomly sampled from $[0,0] \times [10,10]$, with agent goals (9.0, 5.0) and (5.0, 9.0), respectively. The state vector of every agent contains its world frame coordinate $x^{(i)}, y^{(i)}$, and velocity $v_{x^{(i)}}, v_{y^{(i)}}$. The agents' radius is set to $0.5$, and thus safety radius $r=1.0$. The input to each agent's NN control policy is the joint state of the agents, and each agent has its own, potentially different, policy. The collision set is represented as the $L_\infty$ norm ball, i.e. $\mathcal{C}^{(1,2)}=\mathcal{B}_\infty(0, 1)$. With $\mathcal{U} = [-1,-1] \times [1,1]$, we use a single integrator dynamics model,

{\small
    \begin{equation} \label{eq:single_integ}
        \mathbf{x}^{(i)}_{t+1} = 
        \begin{bmatrix}
            \mathbf{I}_2 & \mathbf{0} \\
            \mathbf{0} & \mathbf{0}
        \end{bmatrix}   
        \mathbf{x}^{(i)}_t + 
        \begin{bmatrix}
            \mathbf{I}_2 \\
            \mathbf{I}_2
        \end{bmatrix}
        \mathbf{u}^{(i)}_t.
    \end{equation}
}%

The MSE loss (between NN output and RVO output) of training converged to 0.001 after 20 epochs, indicating the NN policy  encodes the RVO algorithm reasonably well. However, ReBAR is able to identify unsafe regions in this multiagent system, despite the low testing loss. For example, the RBPOA generated by \cref{alg:ReBAR}, with measurement uncertainty $\epsilon^{(1)} = \epsilon^{(2)} = [0.5, 0.5, 0, 0]$, is shown in \cref{fig:two_agent_verify}. The RBPOA shows the two agent system is unsafe, in particular when agent 2 is to the bottom right of agent 1, which matches our intuition because the goal of agent 2 is on the top left of the goal of agent 1. The RBPOA we computed encloses the ground truth relative backprojection set under approximation (RBPUA) from 2M Monte Carlo simulations, succesfully identifying unsafe cases that exhaustive sampling fails to capture and significantly shrinking the relative backreachable set, making it a good reference to be used online for safety verification. \cref{fig:two_agent_verify}(b) shows RBPOAs for 5 timesteps (magenta) and their respective RBPUAs (blue).

\begin{figure}[t]
    \vspace{5pt}
    \captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=0.95\linewidth]{images/experiment/two_agent.png}
    \caption{1 Timestep}
    \end{subfigure}%
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=0.95\linewidth]{images/experiment/5steps.png}
    \caption{5 Timesteps}
    \end{subfigure}
    \caption{(a): RBPOA (magenta), Collision Set (red), Relative Backreachable Set (darkgreen), and RBPUA (blue) obtained by monte-carlo simulation are also shown. (b) Up to 5 step RBPOA, confirmed by sampled RBPUAs.}
    \label{fig:two_agent_verify}
    \vspace{-0.1in}
\end{figure}

Even though this system could not be verified safe everywhere ahead of time (i.e., the RBPOA is not inside the collision set), the system could still be safe in many parts of the state space.
Therefore, we can still provide an online safety check using the RBPOA that was just computed.
In particular, for a given set of initial states (e.g., the current pose estimates of each agent with some uncertainty bounds), we can check whether a collision may be possible collision at the next timestep.
For example, if the two agents' true coordinates are only known to be within the hyper-rectangle $[4, 4.5, 7.5, 3.5] \times [6, 5.5, 9, 4.5]$, ReBAR correctly alerts that a collision could occur in the next timestep. In \cref{fig:online}(a), the unsafe region from Monte Carlo simulation is shown in blue, and is enclosed by the unsafe region (red) generated by solving \cref{eq:online} with coordinates of the agents as the objective function, demonstrating the desired ability of ReBAR to identify unsafe behaviors of a faulty controller. Alternatively, in \cref{fig:online}(b), where the initial states are known to be within $[3, 3, 0.5, 4] \times [4, 4, 1.5, 5]$, \cref{eq:online} is infeasible, and therefore the online check returns that there is no collision possible on the next timestep, which is empirically confirmed by Monte Carlo simulations. Computing the RBPOAs takes $11.2 \pm 0.16$s on average (of 10 experiments), and the online LP takes $1.4 \pm 0.40$ms.

We further provide experiment on a double integrator model. 
The setting remains the same as the previous experiment, except the neural network controller learns to predict the acceleration that matches the agents' velocity with the optimal velocity produced by RVO. The new control signal vector is $[a_{x^{(i)}}, a_{y^{(i)}}] \in [-2, -2] \times [2, 2]$. The double integrator dynamic model we consider is given in \cref{eq:double_integ}. 
Verifying this system takes 9.7 $\pm$ 0.39s, demonstrating our approach's capability of handling more complex dynamics.

{\small
    \begin{equation} \label{eq:double_integ}
        \mathbf{x}^{(i)}_{t+1} = 
        \begin{bmatrix}
            \mathbf{I}_2 & \mathbf{I}_2 & \mathbf{0}_2 & \mathbf{0}_2 \\
            \mathbf{0} & \mathbf{I}_2 & \mathbf{0}_2 & \mathbf{0}_2
        \end{bmatrix}   
        \mathbf{x}^{(i)}_t + 
        \begin{bmatrix}
            0.5\mathbf{I}_2 \\
            \mathbf{I}_2
        \end{bmatrix}
        \mathbf{u}^{(i)}_t.
    \end{equation}
}%

\begin{figure}[t] 
    \vspace{5pt}
    \captionsetup[subfigure]{justification=centering}
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=0.95\columnwidth]{images/experiment/online.png}
    \caption{Successfully identified some starting positions are unsafe}
    \end{subfigure}%
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=0.95\linewidth]{images/experiment/online_safe.png}
    \caption{Successfully verified starting positions are safe}
    \end{subfigure}
    \caption{agent 1 (brown) and agent 2 (olive) state with uncertainty. (a): Unsafe set over approximation (red) encloses unsafe set under approximation (blue). (b): state safe by online safety check, all simulations do not result in collision.}
    \label{fig:online}
    \vspace{-0.1in}
\end{figure} 

